Learning Exhaustive Correlation for Spectral Super-Resolution: Where Spatial-Spectral Attention Meets Linear Dependence

Spectral super-resolution that aims to recover hyperspectral image (HSI) from easily obtainable RGB image has drawn increasing interest in the field of computational photography. The crucial aspect of spectral super-resolution lies in exploiting the correlation within HSIs. However, two types of bottlenecks in existing Transformers limit performance improvement and practical applications. First, existing Transformers often separately emphasize either spatial-wise or spectral-wise correlation, disrupting the 3D features of HSI and hindering the exploitation of unified spatial-spectral correlation. Second, existing self-attention mechanism always establishes full-rank correlation matrix by learning the correlation between pairs of tokens, leading to its inability to describe linear dependence widely existing in HSI among multiple tokens. To address these issues, we propose a novel Exhaustive Correlation Transformer (ECT) for spectral super-resolution. First, we propose a Spectral-wise Discontinuous 3D (SD3D) splitting strategy, which models unified spatial-spectral correlation by integrating spatial-wise continuous splitting strategy and spectral-wise discontinuous splitting strategy. Second, we propose a Dynamic Low-Rank Mapping (DLRM) model, which captures linear dependence among multiple tokens through a dynamically calculated low-rank dependence map. By integrating unified spatial-spectral attention and linear dependence, our ECT can model exhaustive correlation within HSI. The experimental results on both simulated and real data indicate that our method achieves state-of-the-art performance. Codes and pretrained models will be available later.

==> sec/0_abstract.tex <==
\begin{abstract}
Hyperspectral images consist of multiple spectral channels, while spectral super-resolution tasks involve reconstructing hyperspectral images from 3-channel RGB images. Due to the spatial-spectral similarity and redundant information, hyperspectral images exhibit abundant spatial-spectral correlations and mutual linear dependence. However, CNNs with static weights have difficulty capturing these correlations. Moreover, for Transformer models, firstly, existing Transformers for spectral super-resolution only model spectral-wise correlation. While there are some works in other domains that separately model spectral-wise and spatial-wise correlation, these approaches often cannot capture unified correlations effectively. Secondly, the attention mechanisms employed by existing Transformers typically capture full-rank correlation matrices between paired tokens, which cannot model low-rank mutual linear dependence among all tokens. To address these issues, we propose a novel Exhaustive Correlation Transformer (ECT). Firstly, We propose a Spectral-wise Discontinuous 3D (SD3D) token splitting strategy, which simultaneously splits tokens in spatial and spectral dimensions using continuous and discontinuous approaches, enabling the modeling of unified spatial-spectral correlation. Secondly, we propose a Dynamic Low-Rank Mapping (DLRM) model, which can dynamically capture mutual linear dependence among all tokens through a low-rank matrix. The experimental results indicate that our method achieves SOTA, with the lowest loss achieved under the minimal parameters and computational costs. Codes and pretrained models are available at \url{} .
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}


% 1.先验引出，高光谱图像具有空间、谱间相关性；具有线性相关性。
% 2. 建模空间、谱间相关性很重要，但是有低秩约束。Unified Attention Meets Low-Rank Constrain

% 高光谱图像 (HSI）具有多个通道，每个通道表示一个波段的响应。相比于3通道的RGB图像，高光谱图像能更好的记录场景的反射光谱信息。由于这些优势，高光谱图像被广泛应用于遥感、图像分类、目标检测等领域。然而，高光谱图像的采集通常比较困难。推扫式高光谱相机通常需要较长的时间采集一幅场景，这对于采集动态场景、光照变化剧烈的场景都是不利的。此外，高光谱图像信息含量高，会占用更多的存储空间，不利于传输。
Hyperspectral images (HSI) consist of multiple channels, with each channel representing the response in a specific spectral band. Compared to 3-channel RGB images, hyperspectral images excel in capturing detailed spectral information from a scene. Due to these advantages, hyperspectral images find extensive applications in remote sensing~\cite{melgani2004classification,borengasser2007hyperspectral}, image classification~\cite{camps2005kernel,hu2015deep}, object detection~\cite{liang2013salient}, and more. However, acquiring hyperspectral images can be challenging. Pushroom scanners typically require a longer time to capture a scene, which can be disadvantageous for dynamic or rapidly changing scenes. Additionally, hyperspectral images are information-rich, demanding more storage space and making them less suitable for efficient transmission.

\begin{figure}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   % \includegraphics{sec/figs/fig_bubble.pdf}
\includegraphics[width=1.0\linewidth]{sec/figs/bubble_no_lable.pdf}
   \caption{MRAE, FLOPs and Parameters comparisons. The horizontal axis is FLOPs, the vertical axis is MRAE loss, and the circle radius is Parameters. Our Exhaustive Correlation Transformer (ECT) achieves the lowest MRAE loss with the lowest FLOPs and the smallest number of parameters.}
   \label{fig:bubble}
\end{figure}

% 由于高光谱图像中存在大量冗余信息，研究人员提出 snapshot compressive imaging (SCI) systems，将高光谱图像压缩为2D的measurement。其中coded aperture snapshot spectral imaging (CASSI)最为突出且被广泛研究。将SCI系统与重建算法相结合，可以高效获取高光谱图像。但是，CASSI系统造价通常很昂贵，因此，从容易获取的RGB图像重建高光谱图像，也称为光谱超分，成为了一个新的课题。
Due to the presence of substantial redundant information in hyperspectral images, researchers have proposed snapshot compressive imaging (SCI) systems to compress hyperspectral data into 2D measurements. Among these, coded aperture snapshot spectral imaging (CASSI) stands out and has been extensively studied. Combining SCI systems with reconstruction algorithms~\cite{xiong2017hscnn,wang2019hyperspectral,wang2020dnu,cai2022mask,cai2022coarse,cai2022degradation,li2023pixel,dong2023residual,cai2023binarized} allows for efficient retrieval of hyperspectral images. However, CASSI systems are often costly to implement. As a result, the task of reconstructing hyperspectral images from easily obtainable RGB images, known as spectral super-resolution, has emerged as a new challenge.



% 高光谱图像通常是低秩的，一方面， Transformer仅仅建模了Spectral-wise non-local Correlation，对Spatial-wise与Local Correlation缺乏建模，不能完整建模full rank attention。另一方面， 训练良好的Transformer中的Attention Map通常为满秩矩阵，不能建模Low rank Correlation。 

% 高光谱图像本身具有高度空间、谱间相关性，现有光谱超分Transformer仅考虑谱间相关性，忽略了空间相关性。更进一步，相关性存在局部、全局层面上的区别，现有Transformer仅考虑了全局性，忽略了局部相关性建模。由于高度的相关性，高光谱图像存在低秩性，但现有Transformer常常没有考虑到这一点。
%为了解决以上问题，我们提出Exhaustive Correlation Transformer (ECT) 用于建模spectral-wise、spatial-wise、local、non-local以及low-rank correlation。我们提出一种Exhaustive Self-Attention模块(ESA)，在空谱方向同时切分token，获得token cube，达到同时建模空谱相关性的作用。更进一步，我们将ESA模块分为ESA_C和ESA_I两种，分别建模token cube之间和token cube内部的Attention。进一步，我们提出一种Low Rank Mapping模块，通过动态生成的低秩矩阵，将特征图投射到低秩空间，学习低秩特征。

The key point for spectral super-resolution lies in the correlation exploitation among HSI.
Early research employs sparse coding~\cite{arad2016sparse} or A+ based shallow method~\cite{aeschbacher2017defense} for spectral super-resolution. However, they often suffer from limited expressive power and generalization ability, thus failing to achieve satisfactory results.
%In early research, \TODO{Early/Antecedent researches employ xxx for } sparse coding~\cite{arad2016sparse} and shallow learning \TODO{do not use the word 'learning'}~\cite{aeschbacher2017defense} methods were employed for spectral super-resolution, but they often failed to achieve satisfactory results \TODO{Point out the reason. like, but they struggled in high computational burden and complex parameter tuning, thus failed to yield satisfactory results}.
With the expansion of computing power, learning-based methods have made great progress in recent years and become the mainstream solution to spectral super-resolution. Currently, Transformers~\cite{cai2022mst++,wang2023learning} have achieved the SOTA performance for spectral super-resolution, by exploiting the spectral-wise correlation with spectral-wise self-attention mechanisms. However, two kinds of bottlenecks exist that limit performance improvement and practical application. First, existing Transformers predominantly focus on spectral-wise correlation while ignoring spatial-wise correlation in spectral super-resolution. Some works for other related tasks ~\cite{li2023spatial,chen2023activating,wang2022s,liu2023unified} try to model spectral-wise and spatial-wise correlations together, but often with separate network modules. The ignorance and separation destroy the 3D nature of HSI and fail to capture the unified spectral-spatial correlation.
Second, the existing spectral-wise self-attention mechanism always learns the correlation between a pair of spectral bands, \ie tokens in Transformer. The shape of the tokens and the Softmax function results in a full-rank correlation matrix. These characteristics lead to its disability of building the mutual linear dependence among all the tokens.


In this paper, we propose an Exhaustive Correlation Transformer (ECT) to model the unified spatial-spectral attention and mutual linear dependence, both of which we believe are crucial for spectral super-resolution. The first motivation of our method originates from the spatial-spectral similarity in HSI, which brings spatial-spectral correlation. Thus, we propose a Spectral-wise Discontinuous 3D (SD3D) splitting strategy to model the unified attention along the spectral and spatial dimensions simultaneously. This splitting strategy involves continuous splitting in the spatial dimension and discontinuous splitting in the spectral dimension. It allows for a more effective focus on spectral-wise non-local features and does not disrupt the continuous structure in the spatial dimension. 
%\TODO{why spectral-wise, where is the spatial-wise} \TODO{continuous? the name SD3D is Discontinuous}
The second motivation of our methods originates from the information redundancy in HSI, which brings mutual linear dependence. Thus, we propose a Dynamic Low-Rank Mapping (DLRM) module, which first involves interaction between tokens and then maps each token into a low-rank space, thus learning dynamic low-rank correlation matrices, to model the mutual linear dependence among all tokens.
By integrating unified attention with mutual linear dependence, our ECT achieves SOTA performance in extensive synthetic simulation and real experiments.


%Mutual linear dependence is a complex form of correlation that involves the entire set of tokens, resulting in a low-rank correlation matrix for tokens. 
%The low-rank prior induced by linear dependence has been widely studied and applied in spectral reconstruction~\cite{zhang2021learning,zhang2019computational,fu2016exploiting}.
%To model the mutual linear dependence among all tokens, we propose a Dynamic Low-Rank Mapping (DLRM) module. This module interacts and maps each token to a low-rank space, thereby learning dynamic low-rank correlation matrices.
% To address these issues, we propose an Exhaustive Correlation Transformer (ECT) to model spectral-wise, spatial-wise, local, non-local, and low-rank correlation, thus modeling exhaustive correlation for spectral super-resolution. We introduce an Exhaustive Self-Attention (ESA) module that simultaneously divides tokens in spatial and spectral directions, creating a token cube to model spatial-spectral correlations concurrently. Furthermore, we divide the ESA module into two classes: $\rm {ESA_{C(ross)}}$ and $\rm {ESA_{I(nter)}}$, which respectively model attention among tokens and within tokens. Additionally, we propose a Low-Rank Mapping (LRM) module that projects feature maps into a low-rank space, allowing the learning of low-rank features.
%为了解决以上问题，我们提出Exhaustive Correlation Transformer (ECT)，其中的重要模块为Exhaustive

%\TODO{Bellow needs to be polished}

Our contributions are summarized as follows:
\begin{itemize} [leftmargin=0.7cm]
\item We propose a novel Exhaustive Correlation Transformer (ECT) to model spatial-spectral unified correlation and mutual linear dependence, thus modeling exhaustive correlations within hyperspectral images for spectral super-resolution.

\item We propose a Spectral-wise Discontinuous 3D (SD3D) splitting strategy to effectively capture unified spatial-spectral correlation by concurrently adopting spatial-wise continuous and spectral-wise discontinuous splitting.

\item We propose a Dynamic Low-Rank Mapping (DLRM) module, which models the mutual linear dependence within hyperspectral images by dynamically calculating a low-rank correlation matrix among all tokens.
%When combined with Full-Rank Self-Attention (FRSA), it allows for comprehensive modeling of both low-rank and full-rank correlations within hyperspectral images while preserving strong expression power.

\item The experimental results indicate that our method achieves state-of-the-art (SOTA), with the lowest loss achieved under the minimal parameter and computational costs, as shown in Figure ~\ref{fig:bubble}.

\end{itemize}
% Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
% This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

% %-------------------------------------------------------------------------
% \subsection{Language}

% All manuscripts must be in English.

% \subsection{Dual submission}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a
% discussion of the policy on dual submissions.

% \subsection{Paper length}
% Papers, excluding the references section, must be no longer than eight pages in length.
% The references section will not be included in the page count, and there is no limit on the length of the references section.
% For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
% {\bf There will be no extra page charges for \confName\ \confYear.}

% Overlength papers will simply not be reviewed.
% This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
% Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
% The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
% The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

% %-------------------------------------------------------------------------
% \subsection{The ruler}
% The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
% The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
% If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
% The presence or absence of the ruler should not change the appearance of any other content on the page.
% The camera-ready copy should not contain a ruler.
% (\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

% Reviewers:
% note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
% Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


% \subsection{Paper ID}
% Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
% If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


% \subsection{Mathematics}

% Please number all of your sections and displayed equations as in these examples:
% \begin{equation}
%   E = m\cdot c^2
%   \label{eq:important}
% \end{equation}
% and
% \begin{equation}
%   v = a\cdot t.
%   \label{eq:also-important}
% \end{equation}
% It is important for readers to be able to refer to any particular equation.
% Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
% It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
% (Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
% All authors will benefit from reading Mermin's description of how to write mathematics:
% \url{http://www.pamitc.org/documents/mermin.pdf}.

% \subsection{Blind review}

% Many authors misunderstand the concept of anonymizing for blind review.
% Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

% Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
% That is all.
% (But see below for tech reports.)

% Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
% it says that you are building on her work.
% If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

% An example of a bad paper just asking to be rejected:
% \begin{quote}
% \begin{center}
%     An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Removed for blind review
% \end{quote}


% An example of an acceptable paper:
% \begin{quote}
% \begin{center}
%      An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
% \end{quote}

% If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
% In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
% \begin{quote}
% [1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
% \end{quote}

% Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
% For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
% Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
% Then submit the tech report as supplemental material.
% Again, you may not assume the reviewers will read this material.

% Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
% For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
% solution.
% The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

% You can handle this paper like any other.
% Do not write ``We show how to improve our previous work [Anonymous, 1968].
% This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
% That would be silly, and would immediately identify the authors.
% Instead write the following:
% \begin{quotation}
% \noindent
%    We describe a system for zero-g frobnication.
%    This system is new because it handles the following cases:
%    A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
%    Ours handles it by including a foo term in the bar integral.

%    ...

%    The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
%    It displayed the following behaviours, which show how well we solved cases A and B: ...
% \end{quotation}
% As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
% A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
% He or she would have to be sure that no other authors could have been contracted to solve problem B.
% \medskip

% \noindent
% FAQ\medskip\\
% {\bf Q:} Are acknowledgements OK?\\
% {\bf A:} No.  Leave them for the final copy.\medskip\\
% {\bf Q:} How do I cite my results reported in open challenges?
% {\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
% For your results, however, you should not identify yourself and should not mention your participation in the challenge.
% Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%    \caption{Example of caption.
%    It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
%    \label{fig:onecol}
% \end{figure}

% \subsection{Miscellaneous}

% \noindent
% Compare the following:\\
% \begin{tabular}{ll}
%  \verb'$conf_a$' &  $conf_a$ \\
%  \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
% \end{tabular}\\
% See The \TeX book, p165.

% The space after \eg, meaning ``for example'', should not be a sentence-ending space.
% So \eg is correct, {\em e.g.} is not.
% The provided \verb'\eg' macro takes care of this.

% When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
% If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
% However, use it only when there are three or more authors.
% Thus, the following is correct:
%    ``Frobnication has been trendy lately.
%    It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
%    Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

% This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}


==> sec/2_related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\begin{figure*}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   % \includegraphics{sec/figs/fig_bubble.pdf}
\includegraphics[width=1.0\linewidth]{sec/figs/fig_ect.pdf}
   \caption{The macro design of Exhaustive Correlation Transformer (ECT) \TODO{Delete 'ECT' in the figure}}
   \label{fig:ect}
\end{figure*}
\subsection{Spectral Reconstruction}

Hyperspectral image acquisition is typically carried out using push-broom cameras, which can be time-consuming and challenging to capture dynamic scenes or rapidly changing scenes. To address this issue, coded aperture snapshot spectral imaging (CASSI) systems have been widely used, generating 2D measurements~\cite{yuan2021snapshot}, which are then processed through a series of reconstruction algorithms~\cite{xiong2017hscnn,wang2019hyperspectral,wang2020dnu,cai2022mask,cai2022coarse,cai2022degradation,li2023pixel,dong2023residual,cai2023binarized} to obtain hyperspectral images. Due to the presence of substantial redundant information in hyperspectral images, low-rank prior is critical for spectral reconstruction. There are several spectral reconstruction works~\cite{zhang2021learning,zhang2019computational,fu2016exploiting} inspired by the low-rank prior.
% 随着深度学习的发展，卷积神经网络被广泛应用在光谱超分任务上。Shi等人提出一种用于光谱超分的卷积神经网络，取得了NTIRE 2018 Challenge on Spectral Reconstruction from RGB Images的冠军。Li等人将通道注意力机制引入卷积神经网络，提升了性能。
However, CASSI systems are often expensive. Reconstructing hyperspectral images from RGB images is a cost-effective alternative. Arad et al.~\cite{arad2016sparse} employed sparse coding for spectral super-resolution, while Aeschbacher et al.~\cite{aeschbacher2017defense} used shallow learning models and achieved improved results. Three spectral super-resolution challenges ~\cite{arad2016sparse,arad2020ntire,arad2022ntire} were held and significantly inspired the research. With the development of deep learning, convolutional neural networks are widely used in the spectral super-resolution task. Shi et al.~\cite{shi2018hscnn+} proposed a convolutional neural network for spectral super-resolution, which won the NTIRE 2018 Challenge on Spectral Reconstruction from RGB Images. Li et al.~\cite{li2020adaptive,li2022drcr} introduced the channel attention mechanism into the convolutional neural network to improve the performance. Thanks to dynamic weights and long-range correlation modeling, Cai et al.~\cite{cai2022mst++} were the first to introduce Transformers into the field of spectral super-resolution and won first place in the NTIRE 2022 challenge ~\cite{arad2022ntire}.

% With the popularity of deep learning methods, convolutional neural networks have been widely applied in spectral super-resolution~\cite{shi2018hscnn+,li2020adaptive,stiebel2018reconstructing}. Thanks to dynamic weights and long-range correlation modeling, Cai et al.~\cite{cai2022mst++} were the first to introduce Transformers into the field of spectral super-resolution and won the first place in the NTIRE 2022 challenge ~\cite{arad2022ntire}.


\subsection{Transformer Model}

In the field of NLP, to capture long-range dependencies and enable parallel processing, Vaswani et al. ~\cite{vaswani2017attention} introduced the Transformer model based on the self-attention mechanism. Thanks to its capability to capture long-range dependencies, global receptive fields, and dynamic weight computation, Dosovitskiy et al. ~\cite{dosovitskiy2020image} applied the Transformer to image classification, achieving outstanding results. The Transformer architecture has found widespread use in high-level computer vision tasks such as image classification ~\cite{ali2021xcit,yu2022metaformer,chen2021crossvit,li2022efficientformer,liu2021swin}, semantic segmentation ~\cite{strudel2021segmenter,xie2021segformer,lu2021simpler}, and object detection ~\cite{carion2020end,ding2019learning}. Furthermore, in low-level computer vision tasks, Transformer-based models have also demonstrated remarkable performance in tasks like image super-resolution ~\cite{chen2023activating,liang2021swinir,zou2022self,li2023efficient}, deraining ~\cite{zamir2022restormer,xiao2022image,wang2022uformer}, and denoising~\cite{zamir2022restormer,liang2021swinir,wang2022uformer,li2023efficient,zhao2023comprehensive}. Transformers that leverage the self-attention mechanism can capture long-range correlations between Transformer tokens through dot-product similarity calculations and adaptively fuse tokens based on these correlations, offering strong expressive power.

From the perspective of feature maps, token splitting occurs in the spatial~\cite{dosovitskiy2020image,liu2021swin} or spectral dimensions\cite{ali2021xcit,zamir2022restormer,cai2022mst++}, allowing for modeling the relationships between pixels or patches or between channels. While there are some efforts to combine these two types of Transformers to model spatial and spectral correlations~\cite{li2023spatial,chen2023activating,wang2022s,liu2023unified}, most of these works directly treat spatial and spectral Transformers as separate modules, which may not fully capture the unified correlations between spatial and spectral dimensions. However, capturing this kind of correlation is crucial for hyperspectral images.


% All text must be in a two-column format.
% The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
% Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
% The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
% The second and following pages should begin 1 inch (2.54 cm) from the top edge.
% On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
% for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
% page.

% %-------------------------------------------------------------------------
% \subsection{Margins and page numbering}

% All printed material, including text, illustrations, and charts, must be kept
% within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
% high.
% %
% Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
% The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
% The \LaTeX\ template takes care of this when used properly.



% %-------------------------------------------------------------------------
% \subsection{Type style and fonts}

% Wherever Times is specified, Times Roman may also be used.
% If neither is available on your word processor, please use the font closest in
% appearance to Times to which you have access.

% MAIN TITLE.
% Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
% The title should be in Times 14-point, boldface type.
% Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
% do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
% Leave two blank lines after the title.

% AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
% and printed in Times 12-point, non-boldface type.
% This information is to be followed by two blank lines.

% The ABSTRACT and MAIN TEXT are to be in a two-column format.

% MAIN TEXT.
% Type main text in 10-point Times, single-spaced.
% Do NOT use double-spacing.
% All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
% Make sure your text is fully justified---that is, flush left and flush right.
% Please do not place any additional blank lines between paragraphs.

% Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
% Short captions should be centred.

% \noindent Callouts should be 9-point Helvetica, non-boldface type.
% Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

% FIRST-ORDER HEADINGS.
% (For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

% SECOND-ORDER HEADINGS.
% (For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
% If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

% %-------------------------------------------------------------------------
% \subsection{Footnotes}

% Please use footnotes\footnote{This is what a footnote looks like.
% It often distracts the reader from the main flow of the argument.} sparingly.
% Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
% If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
% Use Times 8-point type, single-spaced.


% %-------------------------------------------------------------------------
% \subsection{Cross-references}

% For the benefit of author(s) and readers, please use the
% {\small\begin{verbatim}
%   \cref{...}
% \end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
% This will automatically insert the appropriate label alongside the cross-reference as in this example:
% \begin{quotation}
%   To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
%   It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
%   You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
% \end{quotation}
% If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
% {\small\begin{verbatim}
%   \Cref{...}
% \end{verbatim}}
% command. Here is an example:
% \begin{quotation}
%   \Cref{fig:onecol} is also quite important.
% \end{quotation}

% %-------------------------------------------------------------------------
% \subsection{References}

% List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
% When referenced in the text, enclose the citation number in square brackets, for
% example cite{Authors14}.
% Where appropriate, include page numbers and the name(s) of editors of referenced books.
% When you cite multiple papers at once, please make sure that you cite them in numerical order like this  cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
% If you use the template as advised, this will be taken care of automatically.

% \begin{table}
%   \centering
%   \begin{tabular}{@{}lc@{}}
%     \toprule
%     Method & Frobnability \\
%     \midrule
%     Theirs & Frumpy \\
%     Yours & Frobbly \\
%     Ours & Makes one's heart Frob\\
%     \bottomrule
%   \end{tabular}
%   \caption{Results.   Ours is better.}
%   \label{tab:example}
% \end{table}

% %-------------------------------------------------------------------------
% \subsection{Illustrations, graphs, and photographs}

% All graphics should be centered.
% In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
% Instead use
% {\small\begin{verbatim}
%   \centering
% \end{verbatim}}
% at the beginning of your figure.
% Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
% Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
% Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
% You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.\cite{cai2022mask}

% When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
% {\small\begin{verbatim}
%    \usepackage{graphicx} ...
%    \includegraphics[width=0.8\linewidth]
%                    {myfile.pdf}
% \end{verbatim}
% }


% %-------------------------------------------------------------------------
% \subsection{Color}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

% If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
% Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_method.tex <==
\section{Method}

\begin{figure*}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   % \includegraphics{sec/figs/fig_bubble.pdf}
\includegraphics[width=1.0\linewidth]{sec/figs/fig_esa.pdf}
   \caption{Micro Design of ECT. (a) Exhaustive Self-Attention Block (ESAB). (b) Feed Forward Network (FFN). (c) Exhaustive Self-Attention (ESA) }
   \label{fig:esa}
\end{figure*}

In this section, we will first introduce the macro design of the Exhaustive Correlation Transformer (ECT). Then, we will delve into the micro design within ECT. In this subsection, we detail the crucial model in ECT, the Exhaustive Self-Attention (ESA), and two important models in ESA, the Unified Spatial-Spectral self-Attention (USSA) and the Dynamic Low-Rank Mapping (DLRM).

\subsection{Macro Design}
% 如图1所示，我们提出Exhaustive Correlation Transformer (ECT)。整体网络结构是一个多阶段U形结构，由于上采样和下采样的存在，这种结构可以在减少计算量的同时捕获多尺度空间特征。对于一个3通道的RGB输入，通过一个3×3的卷积将其扩展到31通道，随后送入Ns个U形模块中。每个U形模块包括Embedding、Encoder、bottleneck、decoder和Mapping。embedding和Mapping用3×3卷积实现，分别在输入侧将特征图的通道扩展到32，在输出侧将通道缩减回31.Encoder、Decoder的主体为Cross Exhaustive Self-Attention Block (ESAB)，分别用4×4，stride=2的卷积进行下采样、2×2，stride=2的转置卷积进行上采样。Bottleneck包括一层Inter Exhaustive Self-Attention Block (ESAB)。 特征图的空间分辨率在下采样后变为1/4，通道变为2倍。多头注意力的头数随着通道数的增减成倍增减，初始值为1.Encoder和Decoder之间有残差连接，保留更多的输入信息用于重建。此外添加了一个长距离残差用于稳定训练。ESAB用于建模Token之间的Correlation，ESAB用于建模Token内部的Correlation，分别建模non Local与Local Unified Spatial-spectral correlation。
As shown in Figure ~\ref{fig:ect}, we propose an Exhaustive Correlation Transformer (ECT). The overall network structure is a multi-stage U-shaped architecture, which, thanks to the presence of upsampling and downsampling, can capture multi-scale spatial features while reducing computational costs. For a 3-channel RGB input, it is expanded to 31 channels using a $3\times3$ convolution and then passed through $N_s$ U-shaped modules. Each U-shaped module comprises Embedding, Encoder, Bottleneck, Decoder, and Mapping components. Embedding and Mapping are implemented with $3\times3$ convolutions, expanding the channel dimensions to 32 on the input side and reducing them back to 31 on the output side.
The main components of the Encoder and Decoder are the Cross Exhaustive Self-Attention Blocks (ESAB$\rm {_C}$), utilizing $4\times4$ convolutions with a stride of 2 for downsampling and $2\times2$ transpose convolutions with a stride of 2 for upsampling. The Bottleneck includes a layer of Inter Exhaustive Self-Attention Block (ESAB$\rm {_I}$). ESAB$\rm {_C}$ is employed to model the correlations between tokens, while ESAB$\rm {_I}$ is used to model the correlations within tokens. ESAB$\rm {_C}$ can model spatial-wise non-local and global-aware spectral-wise local correlation, while ESAB$\rm {_I}$ can model spatial-wise local and spectral-wise non-local correlation. The spatial resolution of the feature map becomes $1/4$ after downsampling, while the channel dimensions double. The number of attention heads scales with the channel changes, initially set to 1.
Residual connections exist between the Encoder and Decoder, retaining more input information for reconstruction. Furthermore, a long-range residual connection is added to stabilize training. 

\subsection{Micro Design}
% 由于$\rm {ESAB_{I}}$与$\rm {ESAB_{C}}$的区别仅在于后续处理为Token之间或Token内部，接下来我们以$\rm {ESAB_{C}}$为例介绍Micro Design。
%  如图2所示，一个Exhaustive Self-Attention Block (ESAB)由Exhaustive Self Attention (ESA)、Layer Normalize和Feed Forward Network (FFN)组成。
%  ESA的细节如下：首先，将特征图通过两层分组卷积，学习动态位置编码，然后将位置编码与特征图相加。特征图经过Linear层分别映射到隐空间后，经过3D切分，生成Q、K、V。

% Spatial-wise self-Attention、Spectral-wise Self-Attention以及Exhaustive Self-Attention的Token切分策略对比如图4所示。其中Spatial-wise Self-Attention将一个像素或者一个patch的全部通道视为一个Token，仅建模空间上的相关性。Spectral-wise Self-Attention将每一个通道的全部像素视为一个token，仅建模光谱上的相关性。虽然有一些工作将这两种Attention串联或者并联起来，但是其不能充分挖掘unified spatial-spectral correlation。我们提出的3D切分同时在空间和光谱方向切分token，每个token均包含spatial与spectral局部的信息，通过后面的self-attention建模token之间的correlation，能充分建模unified spatial-spectral correlation。

%假设原特征图的尺寸为$H\times W\times C$，经过3D切分后，Token的数量n为$\frac{C\times s}{c}$，Token的维度d为$\frac{H \times W \times c}{s^2}$，为了简化表达，这里省略多头注意力。Q、K用于建模相关性，首先通过Full-Rank Unified Attention (FRUA)，建模Token两两之间的相关性。然后通过Dynamic Low-Rank Mapping (DLRM)模块，建模mutual Linear Dependence among all tokens。V与FRSA学习到的满秩注意力图相乘，通过Linear层，再与DLRM学到的动态低秩矩阵相乘。进行3D Aline，恢复特征图原本的形状。最后对通道进行shuffle，充分挖掘spectral-wise non-Local特征。


%由于在这里n大于d，以及Softmax的存在，根据~\cite{bhojanapalli2020low}，注意力图降秩的风险较小，学习到的注意力图通常有full rank或high rank。由于full rank注意力图无法表达多个Token之间的线性相关性，我们提出Dynamic Low-Rank Mapping (DLRM)模块，DLRM的细节如图4所示，首先将多头Q、K中的Token进行3D重建，再沿空间维度进行pooling，将Token的空间尺寸从h/s*w/s降为2*2，再通过3d展开将Token恢复为二维矩阵，最后通过一个1d卷积完成各个Head以及各个Token之间的交互，得到一个n*k（k<n）的低秩特征。将Q、K的低秩特征分别进过Softmax约束数据范围，然后转置相乘，得到一个n*n的矩阵，这个矩阵是一个低秩矩阵，其秩不大于k，充分挖掘了mutual Linear dependence among all tokens。
%  FFN由1*1卷积、3*3分组卷积以及GELU激活组成。
% FRSA的表达式如3所示，其中sigma表示Softmax，tau是一个可学习参数。
% Firstly, let's discuss the distinction between ESAB$\rm {_C}$ and ESAB$\rm {_I}$. After the Spectral-wise Discontinuous 3D (SD3D) splitting, each token contains spatial-wise local and spectral-wise non-local information. ESABC is designed to capture correlations between tokens,  while ESABI focuses on modeling correlations within individual tokens.

Since the main difference between ESAB$\rm {_C}$ and ESAB$\rm {_I}$ lies in the subsequent processing, whether it's for correlations between tokens or within tokens, let's focus on ESAB$\rm {_C}$ to illustrate the micro design. Furthermore, from this point onward, we will no longer distinguish between ESAB$\rm {_C}$ and ESAB$\rm {_I}$ in the mathematical notation below.
As depicted in Figure ~\ref{fig:esa}, an Exhaustive Self-Attention Block (ESAB) comprises Exhaustive Self-Attention (ESA), Layer Normalization, and a Feed-Forward Network (FFN). The details of ESA are as follows:

The feature map first undergoes two layers of grouped convolutions to learn dynamic positional encoding. This positional encoding is then added to the feature map.

Then, the feature map is linearly transformed into a hidden space. A Spectral-wise Discontinuous 3D (SD3D) splitting operation is performed to generate $Q$, $K$, and $V$.
% The comparison of the token splitting strategies for Spatial-wise Self-Attention (SpaSA), Spectral-wise Self-Attention (SpecSA), and Exhaustive Self-Attention (ESA) is shown in Figure ~\ref{fig:sa}. SpaSA considers all channels of a pixel or patch as a token, modeling only spatial-wise correlation. SpecSA treats all pixels of each channel as a token, modeling only spectral-wise correlation. Although there are some works~\cite{li2023spatial,chen2023activating,wang2022s,liu2023unified} that connect these two types of Attention in series or parallel, they cannot fully explore the unified spatial-spectral correlation. The SD splitting strategy in ESA divides tokens in both spatial and spectral dimensions using continuous and discontinuous approaches, with each token containing local spatial and non-local spectral information. By modeling the correlation between tokens through self-attention later, ESA can fully model the unified spatial-spectral correlation.


% \begin{figure}[t]
%    \centering
%    % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%     % \includegraphics{sec/figs/fig_bubble.pdf}
%  \includegraphics[width=1.0\linewidth]{sec/figs/fig_sa.pdf}
%     \caption{Token splitting strategy. (a)Spatial-wise Self-Attention. (b)Spectral-wise Self-Attention. (c)Exhaustive Self-Attention}
%     \label{fig:sa}
%  \end{figure}
 
 \begin{figure*}[t]
   \centering
   % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
    % \includegraphics{sec/figs/fig_bubble.pdf}
 \includegraphics[width=1.0\linewidth]{sec/figs/fig_dlrm.pdf}
    \caption{Detailed design of the Dynamic Low-Rank Mapping (DLRM) module.}
    \label{fig:dlrm}
 \end{figure*}

 
If the original feature map has dimensions $H\times W\times C$, after the SD3D splitting, the number of tokens, denoted as $n$, becomes $C\times s/c$, and the dimension of each token, denoted as $d$, becomes $H \times W \times c/s^2$. To simplify the expression, the multi-head attention mechanism is omitted here. $Q$ and $K$ are used to model correlations. First, Unified Spatial-Spectral self-Attention (USSA) is applied to capture independent full-rank correlations between pairs of tokens. The calculation of USSA is expressed by  

\begin{equation}
    {\rm USSA}(Q, K)= \sigma \left(\tau \frac{K^T\times Q}{||K||\cdot||Q||}\right),
    \label{ussa}
\end{equation}

where $\sigma $denotes softmax function and $\tau$ is a learnable parameter. $Q=W_QX$, $K=W_KX$, and $V=W_VX$. Since the dimension of the Token depends on the spatial resolution of the input, 
${\rm L_2}$ normalization is performed within each Token to stabilize the training, and then the expressive power is improved by the learnable parameter $\tau$. Since token dim $d$ is greater than token number $n$ in this scenario, and due to the presence of the Softmax function, there is a lower risk of rank reduction in the attention maps, as discussed in ~\cite{bhojanapalli2020low}. Typically, the learned attention maps have a full rank or nearly full rank. From the optimization point of view, since the linear correlation is different in different hyperspectral images, the loss can only be minimized when the attention mechanism learns full-rank or nearly full-rank attention maps. The experiments confirm this point as well, and we will discuss it in the supplementary material. Furthermore, the scaled dot-product attention is only calculated between paired tokens and cannot capture the mutual linear dependence among all tokens.





% \rm{Softmax}\left(conv\left(pooling\left(K\right) \right)\right)^T \rm{Softmax}\left(conv\left(pooling\left(Q\right) \right)\right) 

To address these issues, we propose the Dynamic Low-Rank Mapping (DLRM) module. 
The details of DLRM are shown in Figure ~\ref{fig:dlrm}. Initially, the tokens from the multi-head Q and K are restored in a 3D manner and then spatially pooled, reducing the spatial dimensions of the tokens from $h/s \times w/s$ to $2\times 2$. Afterward, the tokens are flattened in a 3D manner to restore them to a two-dimensional matrix. Finally, interactions are performed among various heads and tokens through a $1d$ convolution, resulting in a low-rank feature of dimensions $n\times k$ (where $k<n$). The two low-rank features are then passed through the softmax function to limit the data range. The generation of Low-Rank Features (LRFs) can be expressed by 

\begin{equation}
   {\rm LRF}(P)= \sigma\left({\rm conv}\left({\rm pooling}(P)\right), P\in \{Q, K\}\right).
   \label{lrf}
\end{equation} 

 Then they are transposed and multiplied to obtain an adaptive $n\times n$ matrix, which is a low-rank matrix with a rank no greater than $k$.  The calculation of DLRM is expressed by 
 
\begin{equation}
   {\rm DLRM}(Q, K)= {\rm LRF}(K) ^T {\rm LRF}(Q).
   \label{dlrm}
\end{equation}

The difference between the Attention Map in USSA and the Low-Rank Matrix in DLRM is illustrated in Figure ~\ref{fig:lin}. As shown in the figure, the calculation of the correlation in self-attention is token-to-token, where each row of the correlation matrix is independently calculated, and each element in the matrix is only related to two tokens. In contrast, DLRM first facilitates information exchange among various attention heads and tokens. Therefore, each element in the Low-Rank Matrix gathers information from all tokens. Moreover, due to the low-rank nature of the features, the Low-Rank Matrix is low-rank, implicitly modeling the linear correlations among all tokens. In summary, the Low-Rank Matrix can effectively capture the mutual linear dependence among all tokens, which is missing in the Attention Map.


Then $V$ is multiplied by the full-rank attention maps learned by USSA. After passing through a linear layer, it is multiplied by the dynamically learned low-rank matrix from DLRM. The overall arithmetic process of ESA can be summarized by 

\begin{equation}
   {\rm ESA}(X)= {\rm DLRM}(Q,K) \times W \times {\rm USSA}(Q,K)\times V,
   \label{esa}
\end{equation}

 where $W$ is the learnable parameter in the linear layer.
A 3D alignment is then performed to restore the feature map to its original shape. Finally, channel shuffling is applied to fully explore spectral-wise non-local features.

\begin{table*}[h]\small
\caption{The experimental results on the NTIRE 2022 validation dataset are as follows, with \textbf{bold} indicating the first place and \underline{underlined} indicating the second place.}
\label{tab:main_exp}
\centering

\begin{tblr}{
  width=0.9\textwidth,
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {c=2}{},
  cell{1}{4} = {c=2}{},
  cell{1}{6} = {r=2}{},
  cell{1}{7} = {r=2}{},
  % vline{5} = {1}{Black},
  % vline{6} = {2}{Black},
  % vline{7-8} = {10}{Black},
  vline{2,4,6,7} = {-}{0.08em},
  vline{3,5} = {2-11}{0.08em},
  hline{1,11} = {-}{0.1em},
  hline{2} = {2-5}{0.08em},
  hline{3} = {-}{0.1em},
  colspec={X[c]X[c]X[c]X[c]X[c]X[c]X[c]},
  %scale=0.8
}

Method     & \SetCell[c=1]{c} NTIRE 2022 &        & \SetCell[c=1]{c} NTIRE 2020 &        & Params$\downarrow$ & FLOPs$\downarrow$ \\
           & MRAE $\downarrow$      & RMSE$\downarrow$  & MRAE$\downarrow$      & RMSE$\downarrow$  &            &           \\
       
HSCNN+~\cite{shi2018hscnn+}     & 0.3814     & 0.0588 & 0.0684     & 0.0182 & 4.65 M       & 304.45 G    \\
HR Net~\cite{zhao2020hierarchical}     & 0.3476     & 0.0550 & 0.0682     & 0.0179 & 31.70 M      & 163.81 G    \\
AWAN~\cite{li2020adaptive}       & 0.2191     & 0.0349 & 0.0668     & 0.0175 & 4.04 M       & 270.61 G    \\
Restormer~\cite{zamir2022restormer}  & 0.1833     & 0.0274 & 0.0645     & 0.0157 & 15.11 M      & 93.77 G     \\
DRCR~\cite{li2022drcr}   & 0.1823     & 0.0288 & 0.0664     & 0.0171 & 9.48 M       & 586.61 G    \\
MST-L~\cite{cai2022mask}      & 0.1772     & 0.0256 & 0.0646     & 0.0162 & 2.45 M       & 31.82 G     \\
MST++~\cite{cai2022mst++}      & \underline{0.1645}     & \underline{0.0248} & \underline{0.0624}     & \underline{0.0155} & \underline{1.62 M}       & \underline{22.29 G}     \\
\textbf{ECT (Ours)} & \textbf{0.1564}     & \textbf{0.0236} & \textbf{0.0595}     & \textbf{0.0146} & \textbf{1.19 M }      & \textbf{16.75 G}     
\end{tblr}
\end{table*}


Feed Forward Network (FFN) consists of $1\times 1$ convolution, $3\times 3$ grouped convolution and GELU active function. 

\begin{figure}[t]
   \centering
   % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
    % \includegraphics{sec/figs/fig_bubble.pdf}
 \includegraphics[width=1.0\linewidth]{sec/figs/fig_linear_dependent.pdf}
    \caption{Comparison of the Attention Map in USSA and the Low-Rank Matrix in DLRM.}
    \label{fig:lin}
 \end{figure}
 
% You must include your signed IEEE copyright release form when you submit your finished paper.
% We MUST have this form before your paper can be published in the proceedings.

% Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
% \url{https://www.computer.org/about/contact}.


% \end{tabular}
% \end{table*}

==> sec/4_experiments.tex <==
\section{Experiments}
\label{sec:exp}


\subsection{Dataset}
In this paper, we used the NTIRE 2022~\cite{arad2022ntire} and NTIRE 2020 Real World Track~\cite{arad2020ntire} datasets.

The NTIRE 2022 dataset is currently one of the most complex datasets for spectral super-resolution. It was captured using the Specim IQ camera and includes a wide variety of scenes and colors. It was made available for the NTIRE 2022 Spectral Recovery Challenge~\cite{arad2022ntire}. The dataset contains a total of 950 available images, including 900 training images and 50 validation images. The spatial resolution of the images is $482\times 512$, and they consist of 31 spectral channels sampled at 10$nm$ intervals, covering the wavelength range from 400$nm$ to 700$nm$.

The NTIRE 2020 dataset comprises 460 available images, including 450 training images and 10 validation images. The spatial and spectral resolutions of these images are consistent with the NTIRE 2022 dataset.

The process of generating RGB images from the NTIRE 2022 dataset's hyperspectral images is as follows: First, multiply the hyperspectral image of shape $482\times 512 \times 31$ with a Spectral Response Function (SRF) of shape $31\times 3$ to obtain a clean RAW image of shape $482\times 512 \times 3$. Second, add Gaussian Poisson noise to simulate the dark noise and shot noise of the camera sensor, resulting in a noisy RAW image of shape $482\times 512 \times 3$. Third, normalize the mean of the noisy image to 0.18 and apply JPEG compression to obtain the final RGB image. It's important to note that setting the mean value to 0.18 for all RGB images may cause the loss of brightness information from the original scene, making the reconstruction task more challenging. 

The primary difference in the data processing pipeline between NTIRE 2020 and NTIRE 2022 datasets is that NTIRE 2020 applies a mosaic operation to the images before adding noise and then demosaic after adding noise. Additionally, the RGB data in NTIRE 2020 is not normalized to a mean value of 0.18, as is done in NTIRE 2022. Furthermore, the two datasets use different Spectral Response Functions (SRFs). 
%These variations in data processing and characteristics make them distinct datasets, each with its own unique challenges and characteristics.

\begin{figure*}[t]
   \centering
   % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
    % \includegraphics{sec/figs/fig_bubble.pdf}
 \includegraphics[width=1.0\linewidth]{sec/figs/vis_1.pdf}
    \caption{The MRAE loss heatmaps, including 400nm, 500nm, 600nm, and 700nm bands on \textit{ARAD\_0944} from the NTIRE 2022 Validation data.}
    \label{fig:vis1}
 \end{figure*}

\subsection{Implementation Details}
For the hyperparameters in the network structure, we set the SD3D Splitting scale $c=4, s=2$ and low-rank factor $k=12$ for ESAB$\rm {_C}$. For ESAB$\rm {_I}$, we set the SD3D Splitting scale $c=16, s=4$ and low-rank factor $k=8$.
%The hidden dim of a U-shaped net is initially 32.

For the evaluation metrics, following the NTIRE challenge, we evaluate the performance using the Mean Relative Absolute Error  (MRAE) and Root Mean Squared Error (RMSE) metrics.
%, defined as follows:

% \begin{equation}
%     {\rm MRAE}=\frac{1}{N}\sum_{n=1}^N  \frac{\left|I_{GT}^n-I_{Rec}^n\right|}{I_{GT}^n}
%     \label{mrae}
% \end{equation}

% and \TODO{not a new paragraph. Eq.5 and Eq.6 can be deleted or moved to supp.. trivial information}

% \begin{equation}
%     {\rm RMSE} = \sqrt{\frac{1}{N}\sum_{n=1}^N \left ( I_{GT}^n-I_{Rec}^n \right)^2},
%     \label{rmse}
% \end{equation}
% where $I_{GT}^n$ and $I_{Rec}^n$ denote the value of the $n$th pixel in Ground Truth hyperspectral image and reconstructed hyperspectral image. The total number of pixels is $N=H\times W \times C$. 
We primarily use MRAE as the main metric and also adopt it as the training objective.

For the NTIRE 2020 dataset, we use a batch size of 40 and employ a learning rate schedule that follows the Cosine Annealing scheme, decreasing from $4e^{-4}$ to $1e^{-6}$ over $300k$ iterations. We opt for the AdamW optimizer with parameters $\beta_1 =0.9$ and $\beta_2 =0.999$, weight decay is set to $1e^{-4}$. RGB images are first split into $128\times 128$ patches and undergo random rotations and flips for data augmentation before being input into the network. The number of network stages $N_s$ is set to 2.

For the NTIRE 2022 dataset, directly training a 2-stage model is highly unstable. The same issue of instability also persists when training a 3-stage MST++\cite{cai2022mst++} model, with significant differences in training results each time. We have identified several factors contributing to this instability. Firstly, the dataset is characterized by rich and diverse scenes and colors, making model convergence more challenging. Secondly, the RGB data in NTIRE 2022 is mean-normalized, leading to the loss of original scene brightness information, which makes the reconstruction of brightness information difficult and unstable. Additionally, using MRAE as the loss function inherently learns on the ratio between the output and ground truth rather than learning differences. So MRAE loss has a higher frequency than ${\rm L_1}$ or ${\rm L_2}$ loss and is harder to optimize. Lastly, due to the dynamic weights introduced by Transformer models, the training itself can be unstable, and the convergence results highly depend on the initialization of the weight matrices for generating $Q$, $K$, and $V$. To address these challenges, we adopted a two-stage training strategy. First, we trained a 1-stage model with a learning rate that decayed from $5.6e^{-4}$ to $1e^{-6}$ over $200k$ iterations following the Cosine Annealing scheme, using a batch size of 40. Then, the weights of this model were loaded into the first stage of the 2-stage model, and the whole model was trained with a learning rate decaying from $3e^{-4}$ to $1e^{-6}$ over $300k$ iterations follows the Cosine Annealing scheme, again using a batch size of 20. This two-stage training approach helped improve the stability of training on the NTIRE 2022 dataset.

\begin{figure*}[t]
   \centering
   % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
    % \includegraphics{sec/figs/fig_bubble.pdf}
 \includegraphics[width=1.0\linewidth]{sec/figs/vis_2.pdf}
    \caption{The MRAE loss heatmaps, including 400nm, 500nm, 600nm, and 700nm bands on \textit{ARAD\_0940} from the NTIRE 2022 Validation data.}
    \label{fig:vis2}
 \end{figure*}
 
\subsection{Results}
%\TODO{need to supply spectral curve comparison}
\subsubsection{Quantitative Results}
On the NTIRE 2022~\cite{arad2022ntire} and NTIRE 2020~\cite{arad2020ntire} datasets, we compared ECT with various neural networks, as shown in Table ~\ref{tab:main_exp}. HSCNN+ was the champion in the NTIRE 2018 Clean Track and Real World Track. HR Net and AWAN were the champions in the NTIRE 2020 Clean track and Real World track, respectively. DRCR Net and MST++ were the third and first place, respectively, in NTIRE 2022. Restormer is an advanced algorithm in image reconstruction. MST-L is a CASSI-based spectral reconstruction algorithm.  
\subsubsection{Qualitative Results}

 As shown in Figure ~\ref{fig:vis1} and Figure ~\ref{fig:vis2}, we provide qualitative comparisons of MRAE loss heatmaps at 400nm, 500nm, 600nm, and 700nm wavelengths for two images from the NTIRE 2022 Validation dataset. We provide visual effects of the Ground Truth (GT) and MRAE heatmaps for HSCNN+, HR Net, AWAN, Restormer, DRCR Net, MST-L, MST++, and ECT. The visual results indicate that ECT exhibits excellent reconstruction performance across different wavelengths.
 

\subsection{Ablation Study}

All ablation studies are conducted on the NTIRE 2022 dataset with stage $N_s=1$. In each table, \textbf{bold} indicates the first place, and \underline{underlined} represents the second place.


\subsubsection{Ablation Study of SD3D Splitting and DLRM}

The Spectral-wise Discontinuous 3D (SD3D) splitting strategy and the Dynamic Low-Rank Mapping (DLRM) are our two significant contributions. The SD3D splitting strategy is used to model unified spatial-spectral correlation, while DLRM is employed to capture mutual linear dependence. We compared the SD3D splitting strategy and DLRM as ablations with MST++~\cite{cai2022mst++} (stage=1) as the baseline. The experimental results, as shown in Table ~\ref{ab:main}, demonstrate that both the SD3D splitting strategy and DLRM can improve the performance of the baseline. When used together, they achieve even greater performance improvements. It's worth noting that while ECT has higher computational requirements compared to MST++ for a 1-stage model, the 1-stage ECT performs on par with the 3-stage MST++. The 2-stage ECT significantly outperforms the 3-stage MST++.


\begin{table}\small
\caption{Ablation study of the Spectral-wise Discontinuous 3D (SD3D) splitting strategy and the Dynamic Low-Rank Mapping (DLRM) modlue.}
\label{ab:main}
\centering
\begin{tblr}{
  % vline{2,4,6,7} = {-}{0.08em},
  % vline{3,5} = {2-11}{0.08em},
  % hline{1,11} = {-}{0.1em},
  % hline{2} = {2-5}{0.08em},
  hline{1,6} = {-}{0.1em},
  hline{2} = {-}{0.08em},
  colspec={X[c]X[c]X[c]X[c]X[c]X[c]},
}

SD3D & DLRM & MRAE$\downarrow$   & RMSE$\downarrow$   & Params$\downarrow$ & FLOPs$\downarrow$ \\
       \XSolidBrush      &   \XSolidBrush   & 0.1761 & 0.0266 & 0.55M   & 7.84G  \\
    \Checkmark        &   \XSolidBrush   & \underline{0.1700} & \underline{0.0255} & 0.58M   & 8.24G  \\
        \XSolidBrush     & \Checkmark    & 0.1733 & 0.0261 & 0.56M   & 8.27G  \\
     \Checkmark       &  \Checkmark   & \textbf{0.1665} & \textbf{0.0246} & 0.60M   & 8.69G  

\end{tblr}
\end{table}



\begin{table}\small

\caption{Ablation study of the scale of SD3D splitting strategy.}
%\TODO{reduce the font size}
\label{ab:scale}
\centering
\begin{tblr}{
  % vline{2,4,6,7} = {-}{0.08em},
  % vline{3,5} = {2-11}{0.08em},
  % hline{1,11} = {-}{0.1em},
  % hline{2} = {2-5}{0.08em},
  hline{1,8} = {-}{0.1em},
  hline{2} = {-}{0.08em},
  colspec={Q[c]Q[c]X[c]X[c]X[c]X[c]},
}

c & s & MRAE$\downarrow$   & RMSE$\downarrow$   & Params$\downarrow$ & FLOPs$\downarrow$ \\
    1         &  1    & 0.1731 & \textbf{0.0250} & 0.59M   & 8.69G  \\
    32       &   16   & 0.1937 & 0.0285 & 0.94M   & 14.35G  \\
     8        &  4   & 0.1840 & 0.0270 & 0.62M   & 9.49G  \\
     8       &   2  & \underline{0.1709} & 0.0259 & 0.61M   & 8.28G  \\
      4      &   4 & 0.1751 & 0.0264 & 0.66M   & 11.10G  \\
       4      &  2 & \textbf{0.1655} & \textbf{0.0250} & 0.60M   & 8.69G  

\end{tblr}
\end{table}

\subsubsection{Ablation Study on SD3D Splitting Scale}

The important parameters in Spectral-wise Discontinuous 3D (SD3D) splitting are c and s, which control the splitting scale in the spectral and spatial directions, respectively. The ablation study results for c and s in ESAB$\rm {_C}$ are shown in Table ~\ref{ab:scale}. When c = s = 1, it is equivalent to spectral-wise self-attention~\cite{zamir2022restormer}, and when c = 32, s = 16, it is equivalent to spatial-wise self-attention~\cite{dosovitskiy2020image}.



\subsubsection{Ablation Study of Low-Rank Factor $k$}

The critical parameter in DLRM is the number of low-rank feature columns, denoted as $k$. The rank of the dynamic low-rank matrix in DLRM is not greater than $k$. The experimental results for different values of $k$ in ESAB$\rm {_C}$ are shown in Table ~\ref{ab:fac}. When $k = 32$, it means $k = n$, which doesn't constrain the dynamic matrix to be low rank. The experimental results highlight the importance of low rank.

\begin{table}\small

\caption{Ablation study of the low-rank factor $k$.}
\label{ab:fac}
\centering
\begin{tblr}{
  % vline{2,4,6,7} = {-}{0.08em},
  % vline{3,5} = {2-11}{0.08em},
  % hline{1,11} = {-}{0.1em},
  % hline{2} = {2-5}{0.08em},
  hline{1,6} = {-}{0.1em},
  hline{2} = {-}{0.08em},
  colspec={X[c]X[c]X[c]X[c]X[c]},
}

Fac. $k$ & MRAE$\downarrow$   & RMSE$\downarrow$   & Params$\downarrow$ & FLOPs$\downarrow$ \\
   8     & 0.1689 & 0.0260 & 0.60M   & 8.69G  \\
   12   & \textbf{0.1665} & \textbf{0.0246} & 0.60M   & 8.69G   \\
   16     & 0.1671 & 0.0249 & 0.60M   & 8.69G  \\
   32    & 0.1701 & 0.0259  & 0.62M   & 8.69 G  \\

\end{tblr}
\end{table}





%\subsubsection{Ablation Study on Local Correlation}








% \begin{table*}[t]
%   \caption{Experimental results on NTIRE 2022 valid dataset, where bold indicates the first place, underline indicates the second place.}
%   \centering
%   \label{tab:ntire22}
%   \begin{tabular}{lrrrr}
%     \toprule
% Method    & MRAE$\downarrow$    & RMSE$\downarrow$   & Params$\downarrow$  & FLOPs$\downarrow$\\
%     \midrule
% HSCNN+~\cite{shi2018hscnn+}    & 0.3814 & 0.0588  & 4.65 M      & 304.45 G   \\
% HR Net~\cite{zhao2020hierarchical}     & 0.3476 & 0.0550  & 31.70 M      & 163.81 G   \\
% AWAN~\cite{li2020adaptive}     & 0.2191 & 0.0349  & 4.04 M      & 270.61 G   \\

% Restormer~\cite{zamir2022restormer} & 0.1833 & 0.0274  & 15.11 M     & 93.77 G    \\
% DRCR Net~\cite{li2022drcr}   &    0.1823&    0.0288 & 9.48 M     & 586.61 G    \\
% MPR Net~\cite{zamir2021multi}    & 0.1817 & 0.0270  & 3.62 M      & 101.60 G   \\

% MST-L~\cite{cai2022mask}    & 0.1772 & 0.0256  & 2.45 M      & 31.82 G   \\

% % MST++ \textit{Lite}~\cite{cai2022mst++}     & 0.1741 & 0.0269  & 0.55      & 7.84     \\
% % \textbf{HySAT \textit{Lite} (Ours)  }          &0.1656   &\underline{0.0251}  & 0.47 & 7.44 \\
% MST++~\cite{cai2022mst++}     & \underline{0.1645} & \underline{0.0248} & \underline{1.62 M}      & \underline{22.29 G}     \\
% % HySAT  &         \underline{0.1599} & \underline{0.0246}  & \underline{1.40 M}           & \underline{21.08 G}  \\
% %\textbf{HySAT (Ours)}&        \textbf{ 0.1591} & \textbf{0.0248} & \textbf{1.40}           & \textbf{21.08}  \\
% \textbf{ECT (Ours)}& \textbf{0.1569} & \textbf{0.0241}  & \textbf{1.19 M}           & \textbf{16.75 G}  \\
%   \bottomrule
% \end{tabular}
% \end{table*}

% \begin{table}[t]
%   \caption{Experimental results on NTIRE 2020 Real World Track valid dataset, where bold indicates the first place, underline indicates the second place.}
%   \label{tab:ntire20}
%   \begin{tabular}{lrrrr}
%     \toprule
% Method    & MRAE$\downarrow$    & RMSE$\downarrow$  & Params$\downarrow$  & FLOPs$\downarrow$   \\
%     \midrule
% %Stibel~\cite{stiebel2018reconstructing}    & 0.0698 & 0.0187  & \textbf{1.03}  & 63.60\\
% HSCNN+~\cite{shi2018hscnn+}      & 0.0684 & 0.0182  & 4.65 M & 304.44 G\\
% HR Net~\cite{zhao2020hierarchical} & 0.0682 & 0.0179 & 31.70 M & 163.81 G     \\
% AWAN~\cite{li2020adaptive}    & 0.0668 & 0.0175  & 4.04 M& 270.61 G  \\
% DRCR Net~\cite{li2022drcr}   &  0.0664 &  0.0171 & 9.48 M& 586.61 G  \\
% MST-L~\cite{cai2022mask}    & 0.0646 & 0.0162  & 2.45 M      & 31.82 G   \\

% %Restormer~\cite{zamir2022restormer} & 0.0645 & 0.0157  & 15.11 M     & 93.77 G    \\
% %MPR Net~\cite{zamir2021multi}    & 0.0634 & 0.0157  & 3.62 M      & 101.60 G   \\
% MST++~\cite{cai2022mst++}     & \underline{0.0624} & \underline{0.0155}  & \underline{1.62 M} & \underline{22.29 G}    \\ 
% %\textbf{HySAT (Ours)}&  \textbf{0.0598} &   \textbf{0.0142}   & \textbf{1.40 M} & \textbf{21.08 G}      \\

% % HySAT &  \textbf{0.0589} &   \underline{0.0142}   & \underline{1.40 M} & \underline{21.08 G}      \\
% \textbf{ECT (Ours)}&  \textbf{0.0589} &   \textbf{0.0136}   & \textbf{1.19 M} & \textbf{16.75 G}      \\

%   \bottomrule

%   \end{tabular}
% \end{table}

==> sec/5_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this paper, we analyze the limitations of existing Transformers in modeling unified spatial-spectral correlation and mutual linear dependence. We propose a novel Exhaustive Correlation Transformer (ECT) with the key module being Exhaustive Self-Attention (ESA). In ESA, we propose a 3D token splitting strategy to model unified spatial-spectral correlation and a Dynamic Low-Rank Mapping (DLRM) model to capture mutual linear dependence. Experimental results demonstrate that our approach achieves SOTA.

